Impact of Energy Consumption on Multipath TCP Enabled Mobiles

Multiple accesses are common for most mobile devices today. This technological advance opens up a new design space for improving the communication performance of mobile devices. Multipath TCP is a TCP extension that enables using multiple network paths between two end systems for a single TCP connection, increasing performance and reliability. Meanwhile, when operating multiple active interfaces, multipath-TCP also consumes substantial more power and drains out bettery faster than using one interface. Thus, enabling Multipath TCP on mobile devices brings in new challenges. In this paper, we theoretically analyze the underlying design choices given by the Multipath TCP. In particular, we theoretically formulate the rela- tion between performance (throughput) and energy consumption for Multipath TCP. We find that sometime the throughput and energy consumption can be concurrently improved.

==> tex/2_system_model.tex <==












==> tex/3_alg.tex <==
\section{Case I: Real-time Applications}\label{sec:powero}

In this section, we design an energy efficient MP-TCP algorithm for real-time applications. There are two steps in the algorithms: path selection and congestion control. Each source first selects a subset of paths to use and then adapts the rate of each chosen path based on the network congestion. 

For some realtime applications, e.g. video streaming or chatting, the amount of time $T$ for communication is controlled by users. The energy consumption of this type of communication is $T(\sum_{r\in s}P_r(x_r))$. Thus, optimizing energy consumption is equivalent to optimizing power consumption $\sum_{r\in s}P_r(x_r)$. For these applications, we seek to solve 
\begin{subequations}\label{eqn:instantaneous}
\begin{align}
\max \quad& \sum_{s\in \mathcal{S}}\left(U_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}P_r(x_r)\right)\\
\text{s.t.} \quad&  y_l\leq c_l \text{ for }l\in\mathcal{L}
%             \quad &  \sum_{r\in s}x_r\leq \overline x_s
\end{align}
\end{subequations}

We assume for each source $s\in\mathcal{S}$, $U_s(\cdot)$ satisfies C1 and can be interpreted as users' level of satisfaction for the throughput. $\sum_{r\in s}P_r(x_r)$ represents the power consumption. The parameters $\alpha_s\geq 0$ control the tradeoff between users' satisfaction and power consumption. The problem \eqref{eqn:instantaneous} degenerates to \eqref{eqn:umpmax} when $\alpha_s=0$.

Solving \eqref{eqn:instantaneous} is hard because $P_r(x_r)$ is discontinuous at $x_r=0$. In Lemma \ref{lem:nphard} below, we will show that the problem is NP hard even if there is only one source in the network. To tackle the problem efficiently and make it compatible with the current Internet structure, we propose to solve the problem in two steps as follows:

\bee
\item {\it Path Selection}: The source decides a subset of paths $s^*\subseteq s$ to use at the beginning based on available local information, e.g. power characteristics, bandwidth available on each path $r\in s$.
\item {\it Congestion Control}: Once the set $s^*$ of paths is fixed, the source $s$ turns on the interfaces of these paths and adapt rates to network congestion level. 
\eee

Paths should be re-selected from time to time to adapt to changes in power characteristics or available bandwidths, but these conditions usually change at a much slower timescale than congestion level does.  Moreover the switching cost for turning interfaces on and off can be high, further justifying our two-timescale decomposition approach to solving \eqref{eqn:instantaneous}.  We now formally define each subproblem and solve it.



%Since the network conditions sometime will change due to users' mobility and come and go, we can also run path selection in the middle of communication to keep track of the changes, e.g. $(b_r,\theta_r)$. However, the switching cost for turning on/off access interfaces is usually very high so we should avoid doing path selection frequently. This also explains why we decompose the problem \eqref{eqn:instantaneous} into two steps, otherwise we would both need more communication overhead and waste more energy on switching cost due to frequent turning on/off the access. Therefore, although the decomposition may not give a global optimal solution to \eqref{eqn:instantaneous}, it avoids passing of addition information and is compatible with the current Internet. Next, we will formally define the problem we seek to solve in each step and propose an algorithm to solve it.

\subsection{Path Selection}
In this step, each source $s$ selects a subset $s^*\subseteq s$ of paths based on local information, e.g. the available bandwidth $c_r$ of the access link, allocated by the base stations (4G/3G) or the hotspots (WiFi), and the parameters $(b_r,\theta_r)$ in \eqref{eqn:power1} for each path $r\in s$. Then the source $s$ seeks to solve the following problem: 

\noindent {\it Path Selection Problem-I(PSP-I):}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}P_r(x_r)\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

Let the optimal solution to PSP-I be $\bx_s^*$. The paths selected by $s$ are then $s^*=\{r\mid x^*_r>0,r\in s\}$. Comparing PSP-I with the global optimization problem \eqref{eqn:instantaneous}, PSP-I ignores the bandwidth constraints except at the access links. Thus PSP-I provides an upper bound on the throughput. It is a good estimate of the global optimization problem \eqref{eqn:instantaneous} since the access links are usually the bottleneck for most telecommunication standards such as 4G/LTE, WiFi and 3G. 

{\bf Remark}: Various path selection problems are formulated in the literature. In \cite{key2007path}, Key, {\it et al} study the performance of both randomized and game theoretic approach to select a fixed number of paths from a pool of available paths. In \cite{chen2010markov}, the markov approximation approach is proposed for choosing peers in P2P system. Unlike PSP-I, neither of them considers the sunk cost but limits the number of peers one can select to reduce the sunk cost. On the other hand, shortest path routing is a special case of our path selection problem, where, unlike PSP-I, only one path is selected. 

We now characterize an optimal solution to PSP-I in Lemma \ref{lem:optpsp1}.



In Lemma \ref{lem:optpsp1}, we need to compare the objective value of each subset of $s$. Solving PSP-I is in general NP hard because the knapsack problem, which is a well known NP complete problem, can be reduced to PSP-I as shown in Lemma \ref{lem:nphard} below.

\begin{lemma}\label{lem:nphard}
Suppose C1 holds. Then PSP-I is NP hard.
\end{lemma}

However, most mobile devices have only two interfaces (4G and WiFi or 3G and WiFi) and we only need to check each combination in Table \ref{tab:psp1} according to Lemma \ref{lem:optpsp1}.

\begin{table}
\caption{Candidate for PSP-I with $|s|=2$}
\begin{center}
\begin{tabular}{|c|c|}
\hline 
  $x_1$& $x_2$\\
\hline
$\min\{c_1,(U_s')^{-1}(\alpha_sb_1)\}$ & $0$\\
\hline
 $0$ & $\min\{c_2,(U_s')^{-1}(\alpha_sb_2)\}$\\
\hline
$c_1$ & $\min\{\max\{(U_s')^{-1}(\alpha_sb_2)-c_1,0\},c_2\}$\\
\hline
\end{tabular}
\end{center}
\label{tab:psp1}
\end{table}

When there are many WiFi hotspots around, the number $|s|$ of available paths can be larger \cite{wirelessall,wireless1}. Thus PSP-I is hard to be solved efficiently according to Lemma \ref{lem:nphard}. We now propose an efficient heuristic for solving PSP-I that has linear complexity and a provable bound on its suboptimality gap.

First consider the case where $\theta_r=0$ for all $r\in s$ (recall that $\theta_r$ is the sunk power cost of using path $r$), then PSP-I degenerates to a convex program:
\begin{subequations}\label{eqn:simplepsp}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}b_rx_r\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

The KKT conditions implies that the source $s$ uses path $i$ if and only if all the links $j$ with $b_j<b_i$ have been fully used.  Assume without loss of generality $b_i\leq b_j$ for $i<j$. We begin with setting $x_r=0$ for all $r\in s$. We first select path $1$ and calculate the maximum of $U_s(x_1)-\alpha_sb_1x_1$ for $x_1\in[0,c_1]$. We stop if its solution $x_1<c_1$, which means the objective is maximized merely by path 1. Otherwise if $x_1=c_1$, which means the first path is fully utilized, we add path $2$ and calculate maximum of 
$U_s(c_1+x_2)-\alpha_s(b_1c_1+b_2x_2)$ for $x_2\in[0,c_2]$. Again we stop if its solution $x_2<c_2$ and will add path $3$ if $x_2=c_2$. The paths will be added sequentially until $x_k<c_k$ for some $k\leq |s|$ or $k=|s|$. Then the corresponding $\bx_s$ is an optimal solution to \eqref{eqn:simplepsp} and the paths we use are $\{1,\ldots,k\}$.





Theorem \ref{thm:gappsp1} implies that the gap is upper bounded by $\alpha_s\theta_{\hat k}$. It means the algorithm works better when $\theta_k$ are smaller and the gap is closed if there are no sunk costs. The first and second term in the upper bound on the gap $O^* - \hat{O}$ are illustrated in Figure \ref{fig:intuition} as areas A1 and A2 respectively.

In PSP-I, the parameter $\alpha_s$ controls the tradeoff between throughput and energy consumption. Increasing $\alpha_s$ reduces both throughput and power consumption. Although {\bf Algorithm 1} is not guaranteed to obtain an optimal solution to PSP-I, it still has the same property that: {\it Increasing $\alpha_s$ reduces both throughput and power consumption.}

\subsection{Congestion Control}
Once source $s$ fixes the paths $s^*\subseteq s$ it uses, it turns on the access interfaces of the corresponding paths and adapts its rate to network congestion. Similar to the design of congestion control for regular MP-TCP in \cite{pqymptcp}, we need to design $(k_r(\bx_s),\phi_r(\bx_s))$ in \eqref{eqn:TCP_dynamics}-\eqref{eqn:AQM_dynamics}. The power consumption is determined by the steady state throughput of each path, which depends only on $\phi_r(\bx_s)$. We will use the same $k_r(\bx_s)$ as in \cite{pqymptcp}
\bqn
k_r(\bx_s)=\frac{1}{2}x_r(x_r+\|\bx_s\|_{\infty}).
\eqn
Interested readers can refer to \cite[section 4.2]{pqymptcp} for more details. Next, we design $\phi_r(\bx_s)$ for solving \eqref{eqn:instantaneous}. Note that the discontinuity in \eqref{eqn:instantaneous} disappears since the paths for each source is fixed in the path selection step, a standard primal dual decomposition shows that by setting
\bqn
\phi_r(\bx_s)=U'_s(\bfone^T\bx_s)-b_r
\eqn
in \eqref{eqn:TCP_dynamics}-\eqref{eqn:AQM_dynamics} for $r\in s^*$, we obtain a distributed algorithm that converges to an optimal of \eqref{eqn:instantaneous}. This algorithm however is not responsive in a dynamic network because the Hessian of $U_s(\bx_s)$ is only negative semidefinite \cite{boyd2004convex}. To obtain a more responsive algorithm, we multiply a regulation term $f_r(\bx_s)$ in front of $U'_s(\bfone^T\bx_s)$ as we did in \cite{pqymptcp} such that
\bqn
\phi_r(\bx_s)=f_r(\bx_s)U'_s(\bfone^T\bx_s)-b_r,
\eqn
which ensures that the Jacobian of $\Phi_s(\bx_s):=(\phi_r(\bx_s),r\in s)$ is strictly negative definite. We can use the same $f_r(\bx_s)$ as proposed in \cite{pqymptcp}:
\bq\label{eqn:regulation}
f_r(\bx_s)=\beta\frac{\|\bx_s\|_\infty}{x_r}+1-\beta, \quad \beta\in [0,1]
\eq
where a larger $\beta$ gives a more responsive algorithm. It is shown in \cite{pqymptcp} that a more responsive MP-TCP algorithm is less friendly\footnote{Friendliness performance is a metric describing how much MP-TCP flows overtake single-path TCP flows at bottleneck links} to single-path TCP.  The term $f_r(x_s)$ controls the tradeoff between responsiveness and friendliness and a larger $\beta$ yields a more responsive but less friendly algorithm. Here we use $\beta=0.2$ as suggested in \cite{pqymptcp}.


% In \cite{pqymptcp}, it is shown that algorithm with better responsive performance will suffer friendliness performance, a metric describing how much MP-TCP flows overtake single-path TCP flows at bottleneck links. Thus, $f_r(\bx_s)$ controls the tradeoff between responsiveness and fairness performance and larger $f_r(\bx_s)$ gives a more responsive but less friendly algorithm.
%Here, we will use the same parameter $\beta=0.2$ as we did in \cite{pqymptcp}. Interested readers can refer to  \cite[section 4]{pqymptcp} for details.

{\bf Remark:} To the best of our knowledge, all existing MP-TCP algorithms can be modeled by multiplying a regulation term $f_r(\bx_s)$ in front of a marginal utility $U'_s(\bfone^T\bx_s)$, e.g.\cite{Damon,EWTCP}. This improves the responsiveness compared to an algorithm without a regulation term, but effectively modifies the utility function in \eqref{eqn:instantaneous}.  Indeed, for some $f_r(\bx_s)$, the resulting algorithm does not maximize any (modified) utility function \cite{pqymptcp}.

%-----------------------------------------------------------------------------------------------------------------------------
\section{Case II: File Transfer Applications}\label{sec:energybit}

In this section, we design an energy efficient MP-TCP algorithm for file transfer applications. Similar to real-time application, there are two steps in the algorithms: path selection and congestion control. Each source decides a subset of paths to use in the path selection step and adapts rates on the chosen paths to network congestion. 

Unlike realtime application, the size of the data is fixed for file transfer application.
Let the number of bytes be $B$. Then the total energy consumed for source $s$ is $(\sum_{r\in s}P_r(x_r))\frac{B}{\bfone^T\bx_s}$ per transfer. Since $B$ is controlled by the users and can be regarded as a constant, optimizing energy consumption  is equivalent to optimize energy per bit $\frac{\sum_{r\in s}P_r(x_r)}{\bfone^T\bx_s}$. For this type of applications, we seek to solve the following optimization problem
%, which considers user's throughput and the cost of energy per bit compared to \eqref{eqn:umpmax}:
\begin{subequations}\label{eqn:energyperbit}
\begin{align}
\max \quad& \sum_{s\in \mathcal{S}}\left(U_s(\bfone^T\bx_s)-\alpha_s\frac{1}{\bfone^T\bx_s}\sum_{r\in s}P_r(x_r)\right)\\
\text{s.t.} \quad&  y_l\leq c_l \text{ for }l\in\mathcal{L}
      %       \quad &  \sum_{r\in s}x_r\leq \overline x_s
\end{align}
\end{subequations}

where \eqref{eqn:energyperbit} considers both users' satisfaction of the throughput through $U_s(\cdot)$ and the energy per bit for file transfer. Solving \eqref{eqn:energyperbit} is hard not only because of the discontinuity of $P_r(x_r)$ at $x_r=0$, but also the nonconvexity of the fractional $\frac{1}{\bfone^T\bx_s}\sum_{r\in s}P_r(x_r)$. Similar to what we do in section \ref{sec:powero}, we will also decompose the problem into two steps: {\it path selection} and {\it congestion control}.

\subsection{Path Selection}


Similar to path selection in section \ref{sec:powero}, in this step, each source $s$ selects a subset $s^*\subseteq s$ of paths to use based on prior local information, e.g. the available bandwidth $c_r$ and the power throughput characteristic $b_r,\theta_r$ for each path $r\in s$. Then the source $s$ seeks to solve the following problem: 

\noindent {\it Path Selection Problem-II (PSP-II):}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\frac{\alpha_s}{\bfone^T \bx_s}\sum_{r\in s}P_r(x_r)\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}



Compared with PSP-I, PSP-II is not convex even if $P_r(x_r)$ are continuous. However, we will show below that under a mild condition,which covers most existing TCP algorithms, on the utility functions $U_s(\cdot)$, we can solve PSP-II exactly. Again, let $b'_r:=b_r+\theta_r/c_r$. Without loss of generality, $b'_i\leq b'_j$ for $1\leq i< j\leq |s|$. Then {\bf Algorithm 2} solves PSP-II under a mild condition.



For {\bf Algorithm 1}, the sequence $\{O_k,1\leq k\leq |s|\}$ is unimodal and hence the algorithm can stop once the sequence $O_k$ becomes nonincreasing at some $k$. However, this property does not hold for {\bf Algorithm 2} due to the non-convexity of the objective function. Thus, we need to check every element of the sequence $\{O_k,1\leq k\leq |s|\}$. We now show that {\bf Algorithm 2} solves PSP-II under a mild condition C2 below.

\bee
\item [C2]: $x^2U'_s(x)$ is a nondecreasing function of $x$. 
\eee

\begin{theorem}\label{thm:optimal2}
Suppose C1 and C2 hold. Then {\bf Algorithm 2} obtains an optimal solution to PSP-II.
\end{theorem}

For most single-path TCP algorithms, the associated utility function $U_s(\cdot)$ takes the following form
\bq\label{eqn:alphaf}
U_s(x;\alpha)=\gamma\frac{x^{1-\alpha}}{1-\alpha},
\eq
where $\alpha,\gamma\geq 0$ are constants. It is called $\alpha$-fairness function \cite{alpha2000fair} and various TCP algorithms can be recovered by using different $\alpha$ values, e.g. TCP Vegas and FAST correspond to $\alpha=1$ and NewReno corresponds to $\alpha=2$. Since 
\bqn
x^2U'_s(x;\alpha)=\gamma x^{2-\alpha},
\eqn
the $\alpha$-fairness function satisfies C2 when $\alpha\in[0,2]$.

\begin{corollary}
PSP-II can be solved exactly by {\bf Algorithm 2} for TCP algorithms with $\alpha$-fairness utility functions provided $\alpha\in [0,2]$.
\end{corollary}


\subsection{Congestion Control}

Even though the discontinuity disappears once paths $s^*\subseteq s$ we use are fixed, a standard primal dual algorithm  \eqref{eqn:TCP_dynamics}-\eqref{eqn:AQM_dynamics} with 
\bq\label{eqn:primaldual2}
\phi_r(\bx_s)=U'_s(\bfone^T\bx_s)-\alpha_s\frac{\partial E_s(\bx_s)}{\partial x_r}
\eq
where $E_s(\bx_s)=\frac{\sum_{r\in s}P_r(x_r)}{\bfone^T\bx_s}$, can still be unstable since the Hessian is indenifte. As in section \ref{sec:powero}, we use a regulation term $f_r(\bx_s)$ in front of $U'_s(\bfone^T\bx_s)$ to obtain
\bq\label{eqn:energybit}
\phi_r(\bx_s)=f_r(\bx_s)U'_s(\bfone^T\bx_s)-\alpha_s\frac{\partial E_s(\bx_s)}{\partial x_r}
\eq
The regulation term $f_r(\bx_s)$ is merely used to make the algorithm more responsive in section \ref{sec:powero}. Here, it guarantees a stable algorithm, as the following theorem shows. For convenience, we will only prove the result for the following utility function:
\bq\label{eqn:alpha2}
U_s(x)=\frac{2}{\tau^2x},
\eq
where $\tau$ is the round trip time. It corresponds to the utility function of TCP NewReno. Stability can be proved in a similar manner for other utility functions.

\begin{theorem}\label{thm:converge}
For $\phi_r(\bx_s)$ in \eqref{eqn:energybit}, $f_r(\bx_s)$ in \eqref{eqn:regulation}, and $U_s(\cdot)$ in \eqref{eqn:alpha2}, the system \eqref{eqn:TCP_dynamics}-\eqref{eqn:AQM_dynamics} is stable if
\bq\label{eqn:stable1}
\|\bx_s\|_\infty\leq\frac{\beta}{2\alpha_s\tau^2}\frac{9/|s^*|-1}{\max_{r\in s^*}b_r-\min_{r\in s^*}b_r}
\eq
\end{theorem}

\eqref{eqn:stable1} only needs to be satisfied for the selected paths $s^*$. When $\alpha_s$ increases, the size of $s^*$ becomes small, which means $\max_{r\in s^*}b_r-\min_{r\in s^*}b_r$ also decreases. The bound in \eqref{eqn:stable1} is satisfied for most practical scenario. For instance, most of the smartphones have access to both 4G and WiFi, then the bound in \eqref{eqn:stable1} means $\|\bx_s\|_\infty\leq 0.02\frac{\beta}{\alpha_s\tau^2}$ using the medium value in Table \ref{tab:wirelessdata} for $b_r$. In our simulations, $\alpha_s\tau^2$ is typically in $(10^{-5},10^{-3})$. If $\beta=1$, \eqref{eqn:stable1} becomes $\|\bx_s\|_\infty\leq 2000Mbps$ for $\alpha_s\tau^2=10^{-5}$ and $\|\bx_s\|_\infty\leq 20Mbps$ for $\alpha_s\tau^2=10^{-3}$, which seems realistic. The algorithm is always stable in our preliminary simulations.





==> tex/4_discussion.tex <==
\section{Discussions}\label{discussion}

In this section, we evaluate the algorithms developed in section \ref{sec:powero} and \ref{sec:energybit}. In particular, we study the tradeoff between throughput and energy consumption for different parameters $\alpha_s$. We also study the behavior of the energy efficient TCP flows when they interact with regular TCP flows. Finally, we extend the algorithms to cases where there are multiple long term TCP flows from the same device. Unless otherwise specified, we use Table \ref{tab:wirelessdata} for parameter values: For WiFi network, $(c_r,b_r,\theta_r)=$(4.12 Mbps,238.2 mW/Mbps,132.9 mW); for 4G/LTE network, $(c_r,b_r,\theta_r)$=(12.74 Mbps,52 mW/Mbps,1288 mW).


\subsection{Tradeoff between Throughput and Energy Consumption}

We study throughput and energy consumption for both types of applications for different values of $\alpha_s$. Almost all smartphones have both 4G and WiFi access as shown in Figure \ref{fig:cell}.  In the first set of simulations, we assume the bottleneck is at the access link by assuming the bandwidth $c_M$ is very large. Under such scenario, we test the algorithms for both video streaming, which represents realtime application and file download, which represents the file transfer. The simulation results are plotted in Figure \ref{fig:sim1}. For video streaming, we plot the aggregate throughput and power consumption $\sum_{r\in s}P_r(x_r)$ under different values of $\alpha_s$. For file download, we plot the aggregate throughput and the energy per bit $\sum_{r\in s}P_r(x_r)/(\bfone^T\bx_s)$ under different values of $\alpha_s$.



For video streaming, the smartphone uses both 4G and WiFi when $\alpha_s$ is small, it switches to 4G as $\alpha_s$ increases and eventually switch to WiFi network. The aggregate throughput approaches $0$ as $\alpha_s$ increases. Thus, it means there is tradeoff between throughput and energy consumption for realtime application. For file transfer, the smartphone still uses both 4G and WiFi when $\alpha_s$ is small. Different from video streaming, the cell phone always uses 4G network and operates at rate exactly the bandwidth of 4G interface however large $\alpha_s$ is. This means there is no tradeoff between throughput and energy consumption for file transfer application. Actually, we can see that sometimes the smartphone can obtain more throughput as well as reduce energy consumption in section \ref{sec:interaction}.


\begin{lemma}\label{lem:psp111}
Suppose C1 holds. Let $\bx_s^*(\alpha_s)$ be an optimal solution to PSP-I given $\alpha_s$. Then there exists an $\bar \alpha_s>0$ such that when $\alpha_s\geq \bar \alpha_s$, there is only one nonzero element in $\bx_s^*(\alpha_s)$, which can be any element $r_1\in S_1$. In addition, $\lim_{\alpha_s\rightarrow \infty}x_{r_1}^*(\alpha_s)=0$.
\end{lemma}

Lemma \ref{lem:psp111} describes the limiting behavior of realtime application when $\alpha_s$ is large enough. It says that the most energy efficient path is the one with minimal $\theta_r$ for realtime application when $\alpha_s$ is large enough, and the throughput approaches $0$ as $\alpha_s$ increases. 

\begin{lemma}\label{lem:psp222}
Suppose C1 and C2 hold. Let $\bx_s^*(\alpha_s)$ be an optimal solution to PSP-II given $\alpha_s$. Then there exists a $\bar \alpha_s>0$ such that when $\alpha_s\geq \bar \alpha_s$
\bqn
x_r^*(\alpha_s)=\left\{\begin{array}{ll}
0 & r\in s\setminus S_2\\
c_r & r\in S_2
\end{array}\right.
\eqn
\end{lemma}

Lemma \ref{lem:psp222} describes the limiting behavior of file transfer when $\alpha_s$ is large enough. Different from realtime application, its most energy efficient path is the one with minimal $b'_r$ for $\alpha_s$ large enough and it will use all the available bandwidth on paths with minimal $b'_r$.

The above results show the behavior of the algorithm when the bottleneck is at the access part of the smartphone. Sometimes the bottleneck is in the network. We still use Fig. \ref{fig:cell} but assume the bandwidth $c_M=10$Mbps, while the bandwidth of the WiFi and 4G network are 4.12 Mbps and 12.74 Mbps as described in Table \ref{tab:wirelessdata}. If we run regular MP-TCP algorithms, the throughput is 10Mbps and energy per bit is 270.8mJ/Mb. However, if we run the energy efficient algorithms for file transfer, the energy per bit is 194 mJ/Mb for $\alpha\leq 2.4$ and 180.8 mJ/Mb for $\alpha>2.4$  with throughput always being 10 Mbps. Thus, our algorithm can save $33\%$ of the energy compared to regular MP-TCP algorithms without affecting throughput.




\subsection{Interaction with regular TCP flows}\label{sec:interaction}

In this subsection, we study the interaction of our energy efficient TCP flows with regular TCP flows. We will see that sometimes energy efficiency for realtime application and file transfer lead to totally different behaviors. To illustrate, we assume only one path is available for each source now, thus we do not need path selection and will directly do congestion control. The results obtained under multiple paths are similar as discussed below. We evaluate the performance of the algorithms in the network shown in Figure. \ref{fig:cell2}, where an energy efficient TCP flow shares a link with a regular TCP flow. Suppose both the energy efficient TCP and the regular TCP flow use utility function of TCP NewReno, which is $U_s(x):=-\frac{1}{RTT^2x}$ with the same round trip time. 

%We also assume the parameter $(b_r,\theta_r)=(238.2 mW/Mbps,132.9 mW)$, which is the nominal value for WiFi path.

We run the simulations for both video streaming and file download. In Figure \ref{fig:sptcp}, we plot the ratio of the throughput of energy efficient TCP flow to the regular TCP flow for both applications. We find that the ratio tends to be small for video streaming while large for file transfer as $\alpha_s$ increases. The reason behind this is that for realtime application, the energy consumed is proportional to the power $P_r(x_r)=b_rx_r+\theta_r$, which will be reduced when $x_r$ is smaller. However, for file transfer, the energy consumed is proportional to $P_r(x_r)/x_r=b_r+\theta_r/x_r$, which will be reduced when $x_r$ is larger. 



The above results indicate that the energy efficient TCP flow overtakes the regular TCP flow for file transfer applications but undertakes regular TCP flow for realtime applications. When multiple paths are available, the behaviors of these applications are almost unchanged. For realtime application, it ends up at a path in set $S_1$ according to Lemma \ref{lem:psp111} and undertakes the bandwidth at the bottleneck of that path as $\alpha_s$ becomes larger. For file transfer application, it uses all the paths in set $S_2$ according to Lemma \ref{lem:psp222} and overtakes the bandwidth at the bottleneck of those paths as $\alpha_s$ becomes larger.

\subsection{Multiple TCP connections from the same device}



Sometimes there will be multiple long termed TCP connections initiated from the same devices. In this case, we can still run the same congestion control algorithms as described in section \ref{sec:powero} and \ref{sec:energybit} but the path selection algorithms need to be modified. When all of the long termed TCP connections are of the same type, assume them to be realtime applications, each TCP connection has access to the same set of paths and will share the bandwidth equally, thus PSP-I becomes
\begin{subequations}\label{eqn:simplepspN}
\begin{align}
\max \quad& NU_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}b_rx_r\\
\text{s.t.} \quad& x_r\leq \frac{c_r}{N} \quad r\in s
\end{align}
\end{subequations}
where $N$ is the number of TCP connections and can still be solved by {\bf Algorithm 1} by replacing $U_s(\cdot)$ with $N U_s(\cdot)$. {\bf Algorithm 2} can be modified in a similar manner when all the TCP connections are file transfer applications. However, when there are TCP connections of both types of applications, the algorithm is not ready to generalize. Our current approach is that we can run either {\bf Algorithm 1} or {\bf Algorithm 2} assuming all of them are the same type of applications. Our simulation results say that {\bf Algorithm 2} gives a better result most of the time. For example, a smartphone has both 4G and WiFi interfaces as in Figure \ref{fig:cell}. Suppose the smartphone currently has two TCP connections: one video call of duration 5 mins and one file transfer of size 125Mb (1000Mbps). When $\alpha_s=5$, {\bf Algorithm 1} returns the WiFi path while {\bf Algorithm 2} returns the 4G path. In Table \ref{tab:both}, some performance metrics are listed and we see that {\bf Algorithm 2} is better.

\begin{table}
\caption{Comparisons of {\bf Algorithm 1} and {\bf Algorithm 2}.}
\begin{center}
\begin{tabular}{|p{2cm}|p{1.6cm}|p{1.9cm}|p{1.4cm}|}
\hline
 & Throughput of video call  & Completion time of file transfer  & Total energy consumed \\
 \hline
Regular MPTCP&  8.42 Mbps  & 119 s & 794 J \\
 \hline
 Algorithm 1 & 0.40 Mbps& 369  s&  213 J\\
\hline
Algorithm 2 & 0.64 Mbps  &  82.7 s& 161.4 J\\
\hline
\end{tabular}
\end{center}
\label{tab:both}
\end{table}

%-------------------------------------------------
\section{conclusion}\label{conclusion}

In this paper, we design MP-TCP algorithms by jointly considering both throughput and energy consumption for mobile devices. We consider two types of applications: real-time applications, such as video streaming, and file transfer applications, such as file download/upload. We develop energy efficient MP-TCP algorithms for both of them with theoretical performance guarantee. Our preliminary simulation results show that the algorithms can indeed shift traffic to energy efficient path for both two types of application and can reduce energy consumption up to $30\%$ without affecting throughput as compared to baseline MP-TCP algorithm.

There are interesting and future directions that could be explored. It would be useful to generalize the path selection algorithm to the case where there are multiple TCP connections from different types of applications in one device. It is also important to consider switching energy cost when there are numerous small data transfers such as query traffic.


% such as video streaming and file transfer. For applications with numerous small data transfers such as query traffic, we can pack jobs together to avoid switching cost associated with turning on the access interface, but it is beyond the scope of this paper. For applications that involve transferring large volume of data, they typically belong to either of the following two categories:









==> tex/app.tex <==
\appendices

%-------------------------------------------------------------------------------------------------------------------------------------------------------
\section{Proof Sketch of Theorem \ref{thm:gappsp1}}

{\it Proof of Part I}: It can be checked that $O_{i}\leq O_{\hat k-1}$ for $i\leq \hat k-1$ and $O_{i}\leq O_{\hat k}$ for $i\geq k$. Thus by definition of $k^*$, we can obtain the result.

{\it Proof of Part II}: To characterize the gap between the optimal value of PSP-I and objective value given by {\bf Algorithm 1}, we introduce the following optimization problem, which can be regarded as a convex relaxation of PSP-I.

\noindent {\it Relaxation of Path Selection Problem-I(RPSP-I):}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}b'_rx_r\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

{\it RPSP-I} is a convex program obtained by relaxing the noncontinuous $P_r(x_r)$ to $b'_rx_r$. It is hard to evaluate the optimal solution to PSP-I since it is nonconvex, but we can obtain an upper bound of its optimal value by studying RPSP-I. Then we study the gap between this upper bound and the objective value given by {\bf Algorithm 1}.
\begin{lemma}\label{lem:rupperb1}
RPSP-I provides an upper bound for PSP-I problem and its solution $\bx_s^*$ is also optimal to PSP-I if and only if $x_r^*$ is either $0$ or $c_r$ for all $r\in s$.
\end{lemma}

In addition, the optimal solution to RPSP-I is characterized in Lemma \ref{lem:orpsp1}.

\begin{lemma}\label{lem:orpsp1}
Suppose C1 holds. Then $\hat \bx_s$ (defined in \eqref{eqn:optrp}) is an optimal solution to RPSP-I. 
\end{lemma}

By Lemma \ref{lem:rupperb1}, $O^*$ is upper bounded by the optimal value of RPSP-I. By Lemma \ref{lem:orpsp1}, $\hat \bx_s$ is the optimal solution to RPSP-I, thus

\bq\label{eqn:upper2}
O^*\leq U_s(\bfone^T\hat\bx_s)-\alpha_s\sum_{r\in s}b'_r\hat x_r
\eq
Given the bound of $O^*$ in \eqref{eqn:upper2}, we can show that 

\bq\label{eqn:up11}
O^*-O_{\hat k}\leq\alpha_s\theta_{\hat k}(1-\frac{\hat x_{\hat k}}{c_{\hat k}})
\eq
On the other hand,

\bq\label{eqn:up12}
O^*-O_{\hat k-1}\leq\frac{1}{2}\hat x_{\hat k}(U_s'(\hat c)-\alpha_sb'_{\hat k})
\eq

By part I, $k^*\in\{\hat k,\hat k-1\}$, which means the objective value given by {\bf Algorithm 1}: $\hat O=\max\{O_{\hat k}, O_{\hat k-1}\}$. Then substitute \eqref{eqn:up11} and \eqref{eqn:up12}, we can show part II of the theorem.
%-------------------------------------------------------------------------------------------------------
\section{Proof Sketch of Theorem \ref{thm:optimal2}}

To show that {\bf Algorithm 2} obtains the exact optimal solution to PSP-II, we introduce the following optimization problem, which can be seen as the relaxation of PSP-II.

\noindent {\it Relaxation of Path Selection Problem-II (RPSP-II):}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\frac{\alpha_s}{\bfone^T \bx_s}\sum_{r\in s}b'_rx_r\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

\begin{lemma}\label{lem:exactrpsp2}
RPSP-II provides an upper bound for PSP-II problem and its solution $\bx_s^*$ is also optimal to PSP-II if and only if $x_r^*$ is either $0$ or $c_r$ for all $r\in s$.
\end{lemma}

Different from RPSP-I, which is a convex problem, RPSP-II itself is still a nonconvex problem due to the fractional. 
\begin{lemma}\label{lem:optstructure2}
Suppose C1 and C2 hold. Then there exists an optimal solution $\hat\bx_s$ to RPSP-II satisfying
\bq\label{eqn:optrpsp2}
\hat x_i=\left\{\begin{array}{ll}
c_i & i\leq\hat k\\
0 & i>\hat k 
\end{array}\right.
\eq
for some $\hat k\leq |s|$. 
\end{lemma}

In {\bf Algorithm 2}, we compare all the solutions with the structure in \eqref{eqn:optrpsp2}, thus obtain the optimal solution to RPSP-II according to Lemma \ref{lem:optstructure2}, which is also the optimal solution to the original PSP-II based on Lemma \ref{lem:exactrpsp2}.

%-----------------------------------------------------------------------------------------------------------------------------













==> tex/proposal.tex <==
\section{Proposal: Instantaneous Power Minimization}
\todo{Try $2$ route network and get insight. Local path selection algorithm}
\todo{Maximum throughput as a function of the parameter $\alpha_s$.}
\todo{There are tradeoffs between TCP friendliness and Energy Efficiency?}
\todo{Duality Gap of the Power per bit formulation. When strong duality is obtained?}
\todo{Convexification of Energy per bit}
\qiuyu{Model the energy function as a continuous concave function.}


General EEMP-TCP algorithm can be modeled by:
\bqn
\dot x_r=k_r(\bx_s)\left(R_r(\bx_s)\frac{\partial U_s}{\partial x_r}-\alpha_sP'_r(x_r)-q_r\right)_{x_r}^{+},
\eqn
where $R_r(\bx_s)$ is a regulation term and $P_r(x_r)$ is a power cost function.


\subsection{Proposal I}

Then 
The corresponding primal dual algorithm is
\bqn
\dot x_r&=&k_r(\bx_s)\left(\frac{\partial U_s}{\partial x_r}-P'_r(x_r)-\frac{q_r}{2}\right)_{x_r}^{+}\\
&\approx&k_r(\bx_s)\left(\frac{\partial U_s}{\partial x_r}-\frac{P_r(x_r)}{x_r}-\frac{q_r}{2}\right)_{x_r}^{+}
\eqn


\bi
\item Maybe we can use $P_r(x_r)/x_r$ as an approximation of $P'_r(x_r)$.
\item Some applications may have upper bound on the aggregate throughput, e.g. VoIP, video steaming. Then we need to add another constraint for each source $s$: $\sum_{r\in s}x_r\leq \overline x_s$. This can help save energy as well. It means we need to implement a virtual queue in the source or destination.
\item Dummy ACK for downloading job at the mobile device.
\ei

In case the mobile devices downloads, we need to break the dynamics into both source and destination side.
\begin{lemma}\label{lem:approx1}
Suppose function $f(x)$ is convex, increasing and twice differentiable for $x\in[0,\infty)$ with $f(0)=0$. Let $g(x)=\frac{f(x)}{x}$. Then $g(x)$ is also convex, strictly increasing for $x\in[0,\infty)$.
\end{lemma}
Lemma \ref{lem:approx1} shows that if the energy cost $P_r(x_r)$ is a convex increasing function, $P_r(x_r)/x_r$ is a good estimate of $P'_r(x_r)$.

\subsection{Proposal II}
Proposal I even penalizes the route with minimum energy cost. To deal with it, we modify the above algorithm as follows:
\bqn
\dot x_r=k_r(\bx_s)\left(\frac{\partial U_s}{\partial x_r}-(P'_r(x_r)-\min_{k\in s}P'_k(x_k))-\frac{q_r}{2}\right)_{x_r}^{+}
\eqn
When, $P_r(\cdot)$ is linear, there still exists a NUM optimization problem associated with the above algorithm.

\subsection{Proposal III}
We can also express the energy as a constraint in the optimization problem. In this case, we do not need to approximate the marginal energy cost on each route $r$.
\begin{subequations}
\begin{align}
\max \quad& \sum_{s\in S}U_s(\bx_s)\\
\text{s.t.} \quad& H\bx\leq \mathbf{c}\\
%             \quad &  \sum_{r\in s}x_r\leq \overline x_s\\
             \quad &  \sum_{r\in s}P_r(x_r)\leq \overline E_s
\end{align}
$\overline E_s$ is hard to evaluate in reality.
\end{subequations}

\section{Proposal: Power per bit optimization}
\qiuyu{For single-path TCP, this formulation is a convex formulation.}
Maybe it is more convincing to minimize the total energy cost to complete the whole job. In that case, we can also consider the static operation cost. Let the size of the job be $N$, then the energy required to finish it is
\bqn
E_s(\bx_s)=\frac{N}{\|\bx_s\|_1}\sum_{r\in s}P_r(x_r)
\eqn
Then the optimization problem becomes
\begin{subequations}
\begin{align}
\max \quad& \sum_{s\in S}\left(U_s(\bx_s)-\alpha_sE_s(\bx_s)\right)\\
\text{s.t.} \quad& H\bx\leq \mathbf{c}\\
 %            \quad &  \sum_{r\in s}x_r\leq \overline x_s
\end{align}
\end{subequations}
It is a nonconvex optimization problem since $E_s(\bx_s)$ is not concave even if we assume we will use all the subpaths. The Lagrangian is given as
\bqn
L(\bx,\bfp)&=&\sum_{s\in S}\left(U_s(\bx_s)-\alpha_sE_s(\bx_s)\right)-\bfp^T(H\bx-\mathbf{c})\\
&=&\sum_{s\in S}\left(U_s(\bx_s)-\frac{\alpha_s}{\|\bx_s\|_1}\sum_{r\in s}P_r(x_r)-\sum_{r\in s}q_rx_r\right)+\bfp^T\mathbf{c}
\eqn
In general, 
\bqn
\min_{\bfp}\left\{\max_{\bx}\left\{L(\bx,\bfp)\right\}\right\}\geq \max_{\bx}\left\{\min_{\bfp}\left\{L(\bx,\bfp)\right\}\right\}
\eqn
\subsection{A special form of Power consumption}


\section{Path Selection Algorithm}
\subsection{Instantaneous Power Optimization}
For each source $s$, if it has prior knowledge of the bandwidth allocated on each interface, we seek to solve the following combinatorial optimization problem. The formulation is as follows:

\noindent {\it Path Selection Problem-I:}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}P_r(x_r)\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

The greedy algorithm solving {\it Path Selection Problem} is given as follows:
\begin{table}[htbp]
\centering
\normalsize
\begin{tabular}{|p{8.2cm}|}
\hline
{\bf Algorithm 1}: Path Selection Algorithm\\
\hline
{\bf Input}: $U_s(\cdot)$, $\alpha_s$ and $(b_r,\theta_r,c_r)$ for $r\in s$.\\
{\bf Output}: Subset $s'\subseteq s$.\\
\hline
1. Let $z_r:=b_r+\frac{\theta_r}{c_r}$ and label $z_r$ in an ascending order by $\{1,\ldots,|s|\}$ such that $z_i\leq z_j$ for $i\leq j$.\\
2. Calculate $x_k=\min\{(U')^{-1}(\alpha_s b_k),\sum_{i=1}^{k}c_i\}$ and 
\bqn
O_k=U(x_k)-\alpha_s(\sum_{i=1}^{k-1}z_ic_i+\theta_k+b_k(x_k-\sum_{i=1}^{k-1}c_i))
\eqn
3. Let $k^*=\argmax_{1\leq k\leq |s|}\{O_k\}$ and $s'\leftarrow \{1,\ldots,k^*\}$.\\
\hline
\end{tabular}
\end{table}


\begin{lemma}
Suppose condition C1 and C2 hold. Let
\bqn
F_s(\bx_s)&:=&U_s(\bfone^T\bx_s)-\alpha_s\sum_{r\in s}P_r(x_r) \\
f_r(x)&:=&U_s(x)-\alpha_sP_r(x).
\eqn
Then 
\bqn
\max_{\bx_s\geq 0} F_s(\bx_s)=\max_{r\in s}\left\{\max_{x\geq 0} f_r(x)\right\}
\eqn
\end{lemma}
\begin{IEEEproof}
Suppose there exists a $\bx_s^*$ with more than $1$ nonzero entries such that $F_s(\bx_s^*)> \max_{x\geq 0} f_r(x)$ for any $r\in s$. Assume $s=\{1,2,\ldots\}$, $x_1^*,x_2^*>0$ and $f_1(x_1^*+x_2^*)<f_2(x_1^*+x_2^*)$ without loss of generality. Let $\hat \bx_s=(\hat x_1,\hat x_2,\ldots)$ be defined as follows:
\bqn
\hat x_i=\left\{\begin{array}{ll}
x_1^*+x_2^* & i=1\\
0 & i=2\\
x_i^* & \text{otherwise}
\end{array}\right.
\eqn
Then 
\bqn
F_s(\hat\bx_s)-F_s(\bx_s^*)&=&\alpha_s(P_1(x_1^*)+P_2(x_2^*)-P_1(x_1^*+f_2^*))\\
&=&(b_2-b_1)x_2^*+\theta_2\\
&>&\frac{x_2^*\theta_1+x_1^*\theta_2}{x_1^*+x_2^*},
\eqn
where the last inequality follows from $b_2-b_1>\frac{\theta_1-\theta_2}{x_1^*+x_2^*}$ because $f_1(x_1^*+x_2^*)<f_2(x_1^*+x_2^*)$.
\end{IEEEproof}
\begin{corollary}\label{cor:suff1}
For any $\bfq_s\geq 0$, we have
\bqn
\max_{\bx_s\geq 0} (F_s(\bx_s)-\sum_{r\in s}q_rx_r)\leq\max_{r\in s}\left\{\max_{x\geq 0} f_r(x)\right\}
\eqn
\end{corollary}
Corollary \ref{cor:suff1} means if we start with the best path and observe $0$ loss probability, then there is no need to turn on the other interface. A necessary and sufficient certificate is $\frac{\partial U_s(\bfone^T\bx_s)}{\partial x_r}=P'_r(x_r)$.

\begin{lemma}
Suppose $b$ is of ascending order, then the optimal solution to the {\it path selection problem} has the following structure.
For $|s|=2$, the optimal solution is the one of the following combinations that give the largest objective value.
\begin{table}[htdp]
\caption{default}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
 & 1 & 2& 3\\
\hline
$x_1$ & $\min\{c_1,(U')^{-1}(\alpha_sb_1)$ & 0 & $c_1$\\
\hline
$x_2$ & 0 & $\min\{c_2,(U')^{-1}(\alpha_sb_2)\}$ & $\min\{\max\{(U')^{-1}(\alpha_sb_2)-c_1,0\},c_2\}$\\
\hline
\end{tabular}
\end{center}
\label{default}
\end{table}
\end{lemma}

\begin{lemma}\label{lem:gap1}
Suppose $b_r=0$ and define $z_r:=\frac{\theta_r}{c_r}$ for $r\in s$. Without loss of generality, assume $z_r$ is of ascending order. Let the optimal objective value to the {\it path selection problem} be $O^*$ and the objective value given by the greedy algorithm be $\hat O$, then we have 
\bq\label{eqn:gapb}
O^*-\hat O\leq \min\left\{\int_{\sum_{i=1}^{{k^*}-1}c_i}^{(U')^{-1}(z_{k^*})}(U'(y)-\alpha_s z_{k^*-1}y)dy,
\int_{(U')^{-1}(z_{k^*})}^{\sum_{i=1}^{{k^*}}c_i}(\alpha_s z_{k^*}y-U'(y))dy\right\}
\eq
where $k^*:=\max\{k\mid\sum_{i=1}^{k-1}c_i\leq (U')^{-1}(\alpha_s z_k)\}$.
\end{lemma}
\begin{IEEEproof}
Since $b_r=0$ for all $r\in s$, $x_r$ is either $0$ or $c_r$ at optimality. For every subset $s'\subseteq s$, let
\bqn
O(s')=U(\sum_{r\in s'}c_r)-\alpha_s\sum_{r\in s'}\theta_r,
\eqn
which defines the objective value if we choose to use the routes in $s'$. Then the optimal solution to the {\it path selection problem} is $O^*=\max_{s'\subseteq s}\left\{O(s')\right\}$. For $0\leq j\leq |s|$, we define 
\bqn
O_j:=U(\sum_{i=1}^{j}c_i)-\alpha_s\sum_{i=1}^{j}\theta_i=U(\sum_{i=1}^{j}c_i)-\alpha_s\sum_{i=1}^{j}z_ic_i.
\eqn
Based on our greedy algorithm, we have $\hat O=\max\{O_{k^*-1},O_{k^*}\}$. Let $x^*:=(U')^{-1}(\alpha_sz_{k^*})$ and based on definition of $k^*$, we have
\bqn
\sum_{i=1}^{k^*-1}c_i\leq x^*\leq \sum_{i=1}^{k^*}c_i.
\eqn
Let
\bq\label{eqn:upperO}
 \bar O:= U(x^*)-\alpha_s(\sum_{i=1}^{k^*-1}\theta_i+z_{k^*}(x^*-\sum_{i=1}^{k^*-1}c_i)),
\eq
and it is easy to verify that $\min\{\bar O-O_{k^*-1},\bar O-O_{k^*}\}$ is the same as the right side of Eqn.~\eqref{eqn:gapb}. Then we will arrive at our result if we can show that $O^*\leq \bar O$. For every subset $s'=\{k_1,\ldots,k_{|s'|}\}\subseteq s$, we assume $k_1\leq \cdots\leq k_{|s'|}$ without loss of generality. Let
\bqn
\bar h(x):=\left\{\begin{array}{ll}
\alpha_s z_k & \text{if }\exists k\leq k^*-1 \quad\text{s.t. }\quad \sum_{i=1}^{k-1}c_i\leq x<\sum_{i=1}^{k}c_i\\
\alpha_s z_{k^*} & \text{if } \sum_{i=1}^{k^*-1}c_i\leq x<x^* \\
U'(x) & x\geq x^*
\end{array}\right.
\eqn
and 
\bqn
h_{s'}(x):=\left\{\begin{array}{ll}
\alpha_s z_k & \text{if }\exists j\leq |s'| \quad\text{s.t. }\quad \sum_{i=1}^{j-1}c_{k_{i}}\leq x<\sum_{i=1}^{j}c_{k_{i}}\\
U'(x) & x\geq\sum_{i=1}^{|s'|}c_{k_{i}}
\end{array}\right.
\eqn
Next we will show $h(x)\leq h_{s'}(x)$ for $x>0$. Assume $\sum_{i=1}^{|s'|}c_{k_{i}}>x^*$.
For $x\leq x^*$, $\bar h(x)\leq h_{s'}(x)$ since $s'=\{k_1,\ldots,k_{|s'|}\}$ is a subset of $s=\{1,\ldots,|s|\}$. When $x^*\leq x\leq \sum_{i=1}^{|s'|}c_{k_{i}}$, we have
\bqn
\bar h(x)=U'(x)\leq U'(x^*)=\alpha_sz_{k^*}
\eqn
since $U(x)$ is concave by C1. On the other hand, $h_{|s'|}(x)\geq \alpha_sz_{k^*}$ due to the same reason that $s'\subseteq s$. When $x>\sum_{i=1}^{|s'|}c_{k_{i}}$, both $\bar h(x)$ and $h_{|s'|}(x)$ equals $U'(x)$. 
For $\sum_{i=1}^{|s'|}c_{k_{i}}\leq x^*$, we can show that $\bar h(x)\leq h_{|s'|}(x)$ using similar manner. 

For any $0<\epsilon<c_1$, $\bar O$, defined in Eqn.~\eqref{eqn:upperO}, can be rewritten as 
\bqn
\bar O=\int_{\epsilon}^{\infty}(U'(y)-\bar h(y))dy+U(\epsilon)-c_1\epsilon 
\eqn
Similarly, $O(s')$ can be rewritten as 
\bqn
O(s')=\int_{\epsilon}^{\infty}(U'(y)-h_{s'}(y))dy+U(\epsilon)-c_{k_1}\epsilon 
\eqn
Then,
\bqn
\bar O-O(s')=-\int_{\epsilon}^{\infty}(\bar h(y)-h_{s'}(y))dy-(c_1-c_{k_1})\epsilon.
\eqn
Since $\bar h(y)<h_{s'}(y)$ for $y\geq 0$, we have $\bar O-O(s')\geq 0$ for $\epsilon$ small enough. Thus, $\bar O\geq \max_{s'\subseteq s}O(s')=O^*$, which can be used to show Eqn.~\eqref{eqn:gapb} via Eqn.~\eqref{eqn:upperO}.
\end{IEEEproof}
\begin{lemma}\label{lem:optstructure1}
Suppose C1 and C2 hold. Then there exists an optimal solution $\bx_s^*$, where $x_r^*$ is strictly less than $c_r$ for at most one active subpath with $x_r>0$.
\end{lemma}
\begin{IEEEproof}
For any fixed collection of subpaths $s'$, we define the following optimization problem:
\begin{align*}
\max \quad& U_s(\sum_{r\in s'}x_r)-\alpha_s\left(\sum_{r\in s'}b_rx_r+\theta_r\right)\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s'
\end{align*}
which is merely a convex optimization problem, whose Lagrangian can be written as 
\bqn
L(\bx,\mu)&=&U_s(\sum_{r\in s'}x_r)-\alpha_s\left(\sum_{r\in s'}b_rx_r+\theta_r\right)-\sum_{r\in s'}\mu_r(x_r-c_r)\\
&=&U_s(\sum_{r\in s'}x_r)-\sum_{r\in s'}(\alpha_sb_r+\mu_r)x_r-\sum_{r\in s'}(\theta_r-\mu_rc_r).
\eqn
The KKT conditions indicate that, at optimality, for $r\in s'$
\bqn
\frac{\partial U_s(\sum_{r\in s'}x_r)}{\partial x_r}-(\alpha_sb_r+\mu_r)\leq 0,
\eqn
whose equality is obtained if and only if $x_r>0$. Thus, $\alpha_s b_r+\mu_r=\alpha_s b_j+\mu_j$ for all pairs $(r,j)$ with $x_r,x_j>0$. Denote $k:=\argmax_{r\in s'}\{b_r\mid x_r>0\}$. Then we have
\bqn
\mu_r=\alpha_s(b_k-b_r)+\mu_k>0
\eqn
if $x_r>0$ and $b_r<b_k$. Since $\mu_r>0$ indicates $x_r=c_r$ based on KKT conditions, we know that $x_r=c_r$ for all $r\in s'$ such that $b_r<b_k$. Let $\tilde s_k$ be the set of all subpath $r\in s'$ with $b_r=b_k$. Again based on KKT conditions, only their sum $\sum_{r\in \tilde s_k}x_r$ is required to be fixed at $(U')^{-1}(b_k)-\sum_{r:x_r>0}c_r$. Thus, we can construct an optimal solution such that there exists at most one $x_r<c_r$ for $r\in \tilde s_k$. 
\end{IEEEproof}
Now we know for any fixed collection of subpaths $s'$, there exists an optimal solution such that at most one of the $x_r$ is strictly smaller than $c_r$. Since the optimal solution to the {\it path selection problem} can be obtained once we compare all the subsets of $s'$, it means there exists an optimal solution such that at most one of the $x_r$ is strictly smaller than $c_r$ to the {\it path selection problem}.

A generalization of Lemma \ref{lem:gap1} is given below.
\begin{lemma}\label{lem:gap2}
Suppose C1 and C2 hold. Define $z_r:=\frac{\theta_r}{c_r}+b_r$ for $r\in s$. Without loss of generality, assume $z_r$ is of ascending order. Let the optimal objective value to the {\it path selection problem} be $O^*$ and the objective value given by the greedy algorithm be $\hat O$, then we have 
\bq\label{eqn:gapb}
O^*-\hat O\leq \min\left\{\int_{\sum_{i=1}^{{k^*}-1}c_i}^{(U')^{-1}(z_{k^*})}(U'(y)-\alpha_s z_{k^*-1}y)dy,
\int_{(U')^{-1}(z_{k^*})}^{\sum_{i=1}^{{k^*}}c_i}(\alpha_s z_{k^*}y-U'(y))dy\right\}
\eq
where $k^*:=\max\{k\mid\sum_{i=1}^{k-1}c_i\leq (U')^{-1}(\alpha_s z_k)\}$.
\end{lemma}
\begin{IEEEproof}
The proof of Lemma \ref{lem:gap2} can be carried out in a similar manner as Lemma \ref{lem:gap1}. Here we only sketch the proof. 
For any subset $s'\subseteq s$, let
\bqn
\begin{array}{rcl}
O_b(s'):=&\max&\left\{U_s(\sum_{r\in s'}x_r)-\alpha_s\left(\sum_{r\in s'}b_rx_r+\theta_r\right)\right\}\\
&\text{s.t.} & x_r\leq c_r \quad r\in s'
\end{array}
\eqn
Then, we can show $O_{b,j}\geq O_b(s')$ where $s'=\{1,\ldots, j\}$. On the other hand, we can show $\bar O\geq O_b(s')$ for any $s'\subseteq s$. Let $s^*=\{1,\ldots,k^*\}$ be the solution of our algorithm, then we have 
\bqn
O_b(s')-O_b(s^*)\leq \bar O-O_{b,k^*},
\eqn
which is the same upper bound as Eqn.~\eqref{eqn:gapb}.
\end{IEEEproof}






\subsection{Energy Per bit Optimization}

\noindent {\it Path Selection Problem-II (PSP-II):}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\frac{\alpha_s}{\bfone^T \bx_s}\sum_{r\in s}P_r(x_r)\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

\begin{table}[htbp]
\centering
\normalsize
\begin{tabular}{|p{8.2cm}|}
\hline
{\bf Algorithm 2}: Path Selection Algorithm-II\\
\hline
{\bf Input}: $U_s(\cdot)$, $\alpha_s$ and $(b_r,\theta_r,c_r)$ for $r\in s$.\\
{\bf Output}: Subset $s'\subseteq s$.\\
\hline
1. Let $z_r:=b_r+\frac{\theta_r}{c_r}$ and label $z_r$ in an ascending order by $\{1,\ldots,|s|\}$ such that $z_i\leq z_j$ for $i\leq j$.\\
2. Calculate
\bqn
O_k=U_s(\sum_{i=1}^{k}c_i)-\alpha_s\frac{\sum_{i=1}^kz_ic_i}{\sum_{i=1}^{k}c_i}
\eqn
3. Let $k^*=\argmax_{1\leq k\leq |s|}\{O_k\}$ and $s'\leftarrow \{1,\ldots,k^*\}$.\\
\hline
\end{tabular}
\end{table}


\begin{lemma}\label{lem:optstructure2}
Suppose C1 and C2 hold. Then there exists an optimal solution $\bx_s^*$, where $x_r^*$ is strictly less than $c_r$ for at most one active subpath with $x_r>0$.
\end{lemma}
\begin{IEEEproof}
This is a counterpart of Lemma \ref{lem:optstructure1} and can be proved in a similar manner. Note that KKT conditions still serve as a necessary condition for optimal solutions even if when the objective is not concave.
\end{IEEEproof}

Let $z_r:=\frac{\theta_r}{c_r}+b_r$, then define the following optimization problem, which can be regarded as a relaxation of PSP-II.

\noindent {\it Relaxation of Path Selection Problem-II (RPSP-II):}
\begin{subequations}
\begin{align}
\max \quad& U_s(\bfone^T\bx_s)-\frac{\alpha_s}{\bfone^T \bx_s}\sum_{r\in s}z_rx_r\\
\text{s.t.} \quad& x_r\leq c_r \quad r\in s
\end{align}
\end{subequations}

\begin{lemma}
Solving RPSP-II provides an upper bound for PSP-II problem.
\end{lemma}
\begin{IEEEproof}
For every feasible $\bx_s$, we have $\sum_{r\in s}z_rx_r\leq \sum_{r\in s}P_r(x_r)$, thus proves the result.
\end{IEEEproof}

\begin{lemma}
Suppose $U(x)=c\frac{1-\alpha}{x^{1-\alpha}}$, where $c$ is a constant and $0\leq \alpha\leq 2$. There exists an optima $\bx_s^*$ for RPSP-II such that $x_r^*=c_r$ for every active route with $x_r^*>0$.
\end{lemma}
\begin{IEEEproof}
According to Lemma \ref{lem:optstructure2}, there exists an optimal solution $\bx_s^*$, where $x_r^*$ is strictly less than $c_r$ for at most one active subpath with $x_r>0$. Without loss of generality, assume there exists an optima such that for $1\leq i\leq k-1$, $x^*_i=c_i$, $x_k^*\in[0, c_k]$ and $x_i=0$ for $k+1\leq i\leq |s|$. According to KKT condition, the necessary condition for optimality is 
\bqn
&&\frac{\partial U(\sum_{i=1}^{k-1}c_i+x_k)}{\partial x_k}+\alpha_s\frac{\sum_{i=1}^{k-1}z_ic_i+z_kx_k}{(\sum_{i=1}^{k-1}c_i+x_k)^2}-\alpha_s\frac{z_k}{\sum_{i=1}^{k-1}c_i+x_k}=\mu_k\\
\Leftrightarrow && \frac{c+\alpha_s(\sum_{i=1}^{k-1}(z_i-z_k)c_i)}{(\sum_{i=1}^{k-1}c_i+x_k)^2}=\mu_k
\eqn
if $x_k>0$. Note that $\mu_k>0$ only if $x_k=c_k$ and thus the only solution to the above equation is $x_k=0$ or $c_k$ at optimality.
\end{IEEEproof}

\section{Common Knowledge}
\bi
\item  4G/LTE sustain a much faster rate than 3G, even WiFi \cite{4GLTE}.
\item 4G consumes $23$ times of the energy used by WiFi \cite{4GLTE}.
\item Both 4G/3G's power throughput curve seems linear Fig.9,10,11(after minus operation cost)\cite{4GLTE}.
\item 4G's RTT jitter is very small compared with 3G, WiFi. \cite{4GLTE}.
\item Uplink is less energy efficient than downlink. But the amount of downlink jobs dominate uplink jobs.
\item Upload Application: VoIP, Photo upload, Video Chat.
\item The tail energy spent on tail is huge for 3G. \cite{3G-GSM}
\ei


















